Path Polymatrix Games are PPAD-hard

We prove that it is PPAD-hard to compute a Nash equilibrium in a tree polymatrix game with at most twenty actions per player, and path polymatrix game with at most four hundred actions per player. These are the first PPAD hardness results for a game with a constant number of actions per player where the interaction graph is acyclic. Along the way we show PPAD-hardness for finding an $\epsilon$-fixed point of a 2D LinearFIXP instance, when $\epsilon$ is any constant less than $0.5$. This result is tight, since finding a 0.5-fixed point in a 2D LinearFIXP instance is trivial.

==> arxiv/combined_gadgets.tex <==
\newsavebox\const
\begin{lrbox}{\const}
\ifthenelse{\boolean{main}}{
\input 01_introduce_constant.tex
}{
\input 01_introduce_constant.tex
}
\end{lrbox}

\newsavebox\add
\begin{lrbox}{\add}
\ifthenelse{\boolean{main}}{
\input 02_addition.tex           
}{
\input 02_addition.tex           
}
\end{lrbox}

\newsavebox\sub
\begin{lrbox}{\sub}
\ifthenelse{\boolean{main}}{
\input 03_subtraction.tex       
}{
\input 03_subtraction.tex       
}
\end{lrbox}

\newsavebox\mult
\begin{lrbox}{\mult}
\ifthenelse{\boolean{main}}{
\input 04_multiplication.tex
}{
\input 04_multiplication.tex
}
\end{lrbox}

%\begin{center}
\begin{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% top left
\draw (-4, 7.5)  node {\usebox\add};
\node at (-3,4) {\LARGE $g_{a,j} = g_{b,j-1} +^b_{0.1} g_{c,j-1}$};

% top right
\draw (9, 7.5)  node {\usebox\mult};
\node at (10,4) {\LARGE $g_{a,j} = g_{b,j'} *^b_{0.1} c$};

% bottom left
\draw (-4, 0)   node {\usebox\sub};
\node at (-3, -3.5) {\LARGE $g_{a,j} = g_{b,j-1} -^b_{0.1} g_{c,j-1}$};

% bottom right
\draw (9, 0)  node {\usebox\const};
\node at (10,-3.5) {\LARGE $g_{i,j} = c$};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{tikzpicture} 
%\end{center}



==> arxiv/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}


%\newcommand{\PPAD}{\ensuremath{\mathtt{PPAD}}\xspace}

% Sets running headers as well as PDF title and authors
\headers{Path Polymatrix Games are PPAD-hard}{A. Deligkas, J. Fearnley, and R. Savani}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Path Polymatrix Games are PPAD-hard\thanks{A conference version of this paper has appeared at ICALP 2020. This version contains full proofs, a new improved and tight lower bound in Theorem 3.7, and also extends the hardness result to polymatrix games played on paths.
\funding{This work was funded by by EPSRC Grant EP/X039862/1 ``NAfANE: New Approaches for Approximate Nash Equilibria'' and EPSRC Grant EP/W014750/1
``New Techniques for Resolving Boundary Problems in Total Search''.}}}

% Authors: full names plus addresses.
\author{Argyrios Deligkas\thanks{Royal Holloway University of London, UK
  (\email{argyrios.deligkas@rhul.ac.uk}).}
\and John Fearnley\thanks{University of Liverpool, UK 
  (\email{john.fearnley@liverpool.ac.uk}, \email{rahul.savani@liverpool.ac.uk}).}
\and Rahul Savani\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> arxiv/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TIKZ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{ifthen}
\newboolean{main}   

\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usetikzlibrary{matrix,arrows,shapes,positioning,calc,snakes,decorations.markings}
\usetikzlibrary{patterns}

% add the following two lines to your document to get bigger arrows
\usetikzlibrary{arrows.meta}
\tikzset{>={Latex[width=2.5mm,length=2mm]}}

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\definecolor{lavander}{cmyk}{0,0.48,0,0}
\definecolor{violet}{cmyk}{0.79,0.88,0,0}
\definecolor{burntorange}{cmyk}{0,0.52,1,0}

\def\lav{lavander!90}
\def\oran{orange!30}

\tikzstyle{players}=[draw,circle,burntorange, left color=\oran,
                       text=violet,minimum width=1cm]

\tikzstyle{playerssmall}=[draw,circle, minimum width=0.5cm]

\tikzstyle{gate}=[draw,circle,minimum width=1.25cm]

\tikzstyle{rect}=[rectangle] %,draw]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\cellsmall}[2]
%{ 
%\begin{tikzpicture}
%\node[rect, draw=none, inner sep=0cm, minimum width=0.5cm, minimum height=0.5cm] { 
%\begin{tikzpicture}
%\node[draw=none] at (0,0) {$#1$}; 
%\node[draw=none] at (1,1) {$#2$};
%\end{tikzpicture}
%};
%\end{tikzpicture}
%}

\newcommand{\cellsmall}[2]
{ 
\begin{tikzpicture}
\node[rect, draw=none, inner sep=0cm, minimum width=0.5cm, minimum height=0.5cm] { 
\begin{tikzpicture}
\node[draw=none] at (0,0) {$#1$}; 
\node[draw=none] at (1,1) {$#2$};
\end{tikzpicture}
};
\end{tikzpicture}
}

\newcommand{\cellmed}[2]
{ 
\begin{tikzpicture}
\node[rect, draw=none, inner sep=0cm, minimum width=0.5cm, minimum height=0.5cm] { 
\begin{tikzpicture}
\node[draw=none] at (0,0) {\Large $#1$}; 
\node[draw=none] at (1,1) {\Large $#2$};
\end{tikzpicture}
};
\end{tikzpicture}
}

\newcommand{\cell}[2]
{ 
\begin{tikzpicture}
\node[rect, draw=none, inner sep=0cm, minimum width=0.5cm, minimum height=0.5cm] { 
\begin{tikzpicture}
\node[draw=none] at (0,0) {\Large $#1$}; 
\node[draw=none] at (0,0) {\Large $#2$};
\end{tikzpicture}
};
\end{tikzpicture}
}

\newcommand{\collabel}[1]
{ 
\begin{tikzpicture}
\node[rect, draw=none, inner sep=0cm, minimum width=0.25cm, minimum height=0.5cm] {\large #1};
\end{tikzpicture}
}
\newcommand{\zerocell}{\cell{0}{0}}
%\NewDocumentCommand{\zerocell}{\cell{0}{0}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% payoff offset from corners of cell
\pgfmathsetmacro{\os}{0.5}

\newcommand{\payoffs}[4]{ 
	\node[xshift=\os cm,yshift=\os cm] at (m-#1-#2.south west) {\LARGE #3};
	\node[xshift=-\os cm,yshift=-\os cm] at (m-#1-#2.north east) {\LARGE #4};
}
\newcommand{\rowstrategy}[2]{ 
	\node[xshift=-\os cm] at (m-#1-1.west) {\LARGE #2};
}
\newcommand{\colstrategy}[2]{ 
	\node[yshift=\os cm] at (m-1-#1.north) {\LARGE #2};
}
\newcommand{\playersshift}[3]{ 
	\coordinate (tl1) at (m-1-#3.north west);
	\coordinate (tl2) at ($(tl1)+(-1,1.25)$);
	\coordinate (tl3) at ($(tl1)!0.5!(tl2)$);
	\draw[-] (tl1) -- (tl2);
	\node[xshift=-0.2cm, yshift=0.1cm, anchor=east] at (tl3) {\LARGE #1};
	\node[xshift=0.2cm, yshift=0.45cm] at (tl3) {\LARGE #2};
}
\newcommand{\players}[2]{ 
	\playersshift{#1}{#2}{1}
}

